Improving the Robustness of 3D Human Pose Estimation: A Benchmark and Learning from Noisy Input

Despite the promising performance of current 3D human pose estimation techniques, understanding and enhancing their generalization on challenging in-the-wild videos remain an open problem. In this work, we focus on the robustness of 2D-to-3D pose lifters. To this end, we develop two benchmark datasets, namely Human3.6M-C and HumanEva-I-C, to examine the robustness of video-based 3D pose lifters to a wide range of common video corruptions including temporary occlusion, motion blur, and pixel-level noise. We observe the poor generalization of state-of-the-art 3D pose lifters in the presence of corruption and establish two techniques to tackle this issue. First, we introduce Temporal Additive Gaussian Noise (TAGN) as a simple yet effective 2D input pose data augmentation. Additionally, to incorporate the confidence scores output by the 2D pose detectors, we design a confidence-aware convolution (CA-Conv) block. Extensively tested on corrupted videos, the proposed strategies consistently boost the robustness of 3D pose lifters and serve as new baselines for future research.

==> sections/dataset_viz.tex <==
\begin{figure*}[t!]
    \pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}
    \pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.5ex}}
    \centering
    
        \hspace{-10pt}
        \begin{tikzpicture}
        \def \h{2.15}
        \def \w{2.10}
        \def \imgw{2.0cm}
        \def \y{0} 
        
        \def \r{0} 
        \node at (-1.5, 0,\h * \r) [below, rotate=90] {\footnotesize{Motion Blur}};
        \node at (-1.5, \h * 1, \h * \r) [below, rotate=90] {\footnotesize{Impulse Noise}};
        \node at (-1.5, \h * 2, \h * \r) [below, rotate=90] {\footnotesize{Gaussian Noise}};
        \node at (-1.5, \h * 3,  \h * \r) [below, rotate=90] {\footnotesize{Cropping}};
        \node at (-1.5, \h * 4,  \h * \r) [below, rotate=90] {\footnotesize{GPE}};
        \draw (\w * 0, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_1.png}};
        \draw (\w * 1, \h * \r)node[inner sep=0]  {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_2.png}};
        \draw (\w * 2, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_3.png}};
        \draw (\w * 3 ,\h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_4.png}};
        \draw (\w * 4, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_5.png}};
        \draw (\w * 5, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_6.png}};
        \draw (\w * 6, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_7.png}};
        \draw (\w * 7, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/motion_blur_8.png}};
        
        \def \r{1} 
        \draw (\w * 0, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_1.jpg}};
        \draw (\w * 1, \h * \r)node[inner sep=0]  {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_2.jpg}};
        \draw (\w * 2, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_3.png}};
        \draw (\w * 3 ,\h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_4.png}};
        \draw (\w * 4, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_5.png}};
        \draw (\w * 5, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_6.png}};
        \draw (\w * 6, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_7.png}};
        \draw (\w * 7, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/impulse_noise_8.png}};
        
        \def \r{2} 
        \draw (\w * 0, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_1.png}};
        \draw (\w * 1, \h * \r)node[inner sep=0]  {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_2.png}};
        \draw (\w * 2, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_3.png}};
        \draw (\w * 3 ,\h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_4.png}};
        \draw (\w * 4, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_5.png}};
        \draw (\w * 5, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_6.png}};
        \draw (\w * 6, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_7.png}};
        \draw (\w * 7, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/gaussian_noise_8.png}};
        
        \def \r{3} 
        \draw (\w * 0, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_1.png}};
        \draw (\w * 1, \h * \r)node[inner sep=0]  {\includegraphics[width=\imgw]{resources/dataset_samples/crop_2.png}};
        \draw (\w * 2, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_3.png}};
        \draw (\w * 3 ,\h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_4.png}};
        \draw (\w * 4, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_5.png}};
        \draw (\w * 5, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_6.png}};
        \draw (\w * 6, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_7.png}};
        \draw (\w * 7, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/crop_8.png}};
        
        \def \r{4} 
        \draw (\w * 0, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_1.png}};
        \draw (\w * 1, \h * \r)node[inner sep=0]  {\includegraphics[width=\imgw]{resources/dataset_samples/erase_2.png}};
        \draw (\w * 2, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_3.png}};
        \draw (\w * 3 ,\h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_4.png}};
        \draw (\w * 4, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_8.jpg}};
        \draw (\w * 5, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_6.png}};
        \draw (\w * 6, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_7.png}};
        \draw (\w * 7, \h * \r) node[inner sep=0] {\includegraphics[width=\imgw]{resources/dataset_samples/erase_5.png}};
        
        
        
        
        \end{tikzpicture}
    \caption{Examples of H36M-C (first five columns from the left) and HumanEva-I-C (last three columns from the left) dataset. Each row corresponds to samples obtained under different video corruption operators.}
    \vspace*{-\baselineskip}
    \label{fig:dataset}
\end{figure*}


==> tables/mpjpe_litehrnet_ca-conv.tex <==
\begin{table*}[t!]
  \caption{Effect of CA-Conv block on $\text{MPJPE}_{\leq 0.1}$ of VP3D\cite{pavllo2019_videopose3d} models trained/tested on 2D keypoints detected by HRNet \cite{sun2019_hrnet} and Lite-HRNet \cite{yu2021_lite-hrnet}.}
  \label{tab:supp_mpjpe_ca-conv-hrnet-lite-hrnet}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}c|c|l|cccccc|c@{}}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Keypoints \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Testing \\ Keypoints \end{tabular}} & \multicolumn{1}{c|}{ \textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impulse \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temporal-patch \\ Erasing\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Guided-patch \\ Erasing\end{tabular}} & \textbf{Cropping} & \textbf{\begin{tabular}[c]{@{}c@{}}Motion \\ Blur\end{tabular}} & \textbf{Average} \\ \midrule
    HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}     
       & $73.11 $ & $74.03 $ & $81.65 $ & $90.56 $ & $79.76 $ & $68.40 $ & $77.92 $ 
    \\
    HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}+{CA-Conv}
       & $72.31 $ & $73.28 $ & $79.45 $ & $87.72 $ & $76.84 $ & $67.16 $ & $76.13 $
    \\
    
    \midrule
    
    HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}
       & $105.71 $ & $109.93 $ & $101.01 $ & $107.46 $ & $83.36 $ & $80.71 $ & $98.03 $ 
    \\
    HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}+{CA-Conv}
        & $107.72 $ & $111.27 $ & $101.56 $ & $107.20 $ & $83.92 $ & $84.17 $ & $99.31 $ 
    \\
    
    \hline
    \midrule
    
    Lite-HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}
        & $78.21 $ & $80.34 $ & $87.56 $ & $97.35 $ & $89.27 $ & $71.77 $ & $84.08 $ 
    \\
    Lite-HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}+{CA-Conv}
        & $75.24 $ & $77.49 $ & $84.49 $ & $93.92 $ & $88.86 $ & $69.52 $ & $81.59 $ 
    \\
    
    \midrule
    
    Lite-HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}
        & $91.60 $ & $91.89 $ & $97.96 $ & $103.43 $ & $86.79 $ & $79.12 $ & $91.80 $ 
    \\
    Lite-HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}+{CA-Conv}
        & $88.24 $ & $88.31 $ & $95.35 $ & $100.66 $ & $84.97 $ & $76.51 $ & $89.01 $
    \\
    \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/mpjpe_litehrnet_tagn.tex <==
\begin{table*}[t!]
  \caption{Effect of TAGN on $\text{MPJPE}_{\leq 0.1}$ of VP3D \cite{pavllo2019_videopose3d} models trained/tested on 2D keypoints detected by HRNet\cite{sun2019_hrnet} and Lite-HRNet \cite{yu2021_lite-hrnet}. The mean and standard deviations across $5$ random runs are reported.}
  \label{tab:supp_mpjpe_tagn-hrnet-lite-hrnet}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}c|c|l|cccccc|c@{}}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ Keypoints \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Testing \\ Keypoints \end{tabular}} & \multicolumn{1}{c|}{ \textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impulse \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temporal-patch \\ Erasing\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Guided-patch \\ Erasing\end{tabular}} & \textbf{Cropping} & \textbf{\begin{tabular}[c]{@{}c@{}}Motion \\ Blur\end{tabular}} & \textbf{Average} \\ \midrule
    HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}     
        &  94.27& 96.64 & 99.32 & 116.54 & 118.08 &  78.14 & 100.50
    \\
    HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}+{TAGN}
        & $86.30 \pm 0.27$ & $88.46 \pm 0.27$ & $92.57 \pm 0.33$ & $106.74 \pm 0.65$ & $107.71 \pm 0.54$ & $75.89 \pm 0.16$ & $92.94 \pm 0.37$
    \\
    
    \midrule
    
    HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}
        & $123.69$ & $127.27$ & $118.76$ & $132.68$ & $116.56$ & $91.76$ & $118.45$ 
    \\
    HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}+{TAGN}
        & $121.78 \pm 0.25$ & $125.04 \pm 0.28$ & $110.21 \pm 0.36$ & $121.85 \pm 0.73$ & $107.11 \pm 0.76$ & $87.59 \pm 0.16$ & $112.26 \pm 0.42$
    \\
    
    \hline
    \midrule
    
    Lite-HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}
        & $94.32 $ & $96.76 $ & $101.47 $ & $118.77 $ & $121.07 $ & $77.56 $ & $101.66 $ 
    \\
    Lite-HRNet & HRNet & VP3D\cite{pavllo2019_videopose3d}+{TAGN}
        & $91.73 \pm 0.30$ & $94.12 \pm 0.32$ & $96.08 \pm 0.38$ & $112.72 \pm 0.56$ & $117.23 \pm 1.09$ & $76.54 \pm 0.24$ & $98.07 \pm 0.48$ 
    \\
    
    \midrule
    
    Lite-HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}
        & $120.30 $ & $123.76 $ & $116.66 $ & $130.20 $ & $116.80 $ & $87.94 $ & $115.94 $ 
    \\
    Lite-HRNet & Lite-HRNet & VP3D\cite{pavllo2019_videopose3d}+{TAGN}
        & $85.82 \pm 0.33$ & $88.05 \pm 0.33$ & $95.73 \pm 0.24$ & $110.03 \pm 0.30$ & $109.13 \pm 1.05$ & $76.19 \pm 0.17$ & $94.16 \pm 0.40$ 
    \\
    
    \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/mpjpe_receptive_field_ca-conv.tex <==
\begin{table*}[t!]
  \caption{Effect of VP3D \cite{pavllo2019_videopose3d}'s receptive field on $\text{MPJPE}_{\leq 0.1}$ of VP3D models trained with CA-Conv}
  \label{tab:supp_mpjpe-ca-conv-receptive-field}
  \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{@{}c|l|cccccc|c@{}}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Receptive \\ Field \end{tabular}} & \multicolumn{1}{c|}{ \textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impulse \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temporal-patch \\ Erasing\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Guided-patch \\ Erasing\end{tabular}} & \textbf{Cropping} & \textbf{\begin{tabular}[c]{@{}c@{}}Motion \\ Blur\end{tabular}} & \textbf{Average} \\ \midrule
    1 & VP3D\cite{pavllo2019_videopose3d}     
         & $86.96 $ & $87.96 $ & $87.75 $ & $96.52 $ & $81.05 $ & $76.61 $ & $86.14 $
    \\
    1 & VP3D \cite{pavllo2019_videopose3d} + {CA-Conv}
       & $85.21 $ & $86.16 $ & $84.16 $ & $92.16 $ & $77.14 $ & $74.85 $ & $83.28 $ 
    \\
    \hline
    9 & VP3D\cite{pavllo2019_videopose3d}     
        & $78.11 $ & $79.27 $ & $85.68 $ & $94.57 $ & $83.53 $ & $71.92 $ & $82.18 $ 
    \\
    9 & VP3D \cite{pavllo2019_videopose3d} + {CA-Conv}
        & $76.68 $ & $77.58 $ & $82.96 $ & $91.61 $ & $79.53 $ & $69.92 $ & $79.71 $ 
    \\
    \hline
    27 & VP3D\cite{pavllo2019_videopose3d}     
        & $73.11 $ & $74.03 $ & $81.65 $ & $90.56 $ & $79.76 $ & $68.40 $ & $77.92 $ 
    \\
    27 & VP3D \cite{pavllo2019_videopose3d} + {CA-Conv}
        & $72.31 $ & $73.28 $ & $79.45 $ & $87.72 $ & $76.84 $ & $67.16 $ & $76.13 $ 
    \\
    \hline
    81 & VP3D\cite{pavllo2019_videopose3d}     
        & $70.85 $ & $71.82 $ & $79.55 $ & $87.83 $ & $77.94 $ & $66.78 $ & $75.80 $ 
    \\
    81 & VP3D \cite{pavllo2019_videopose3d} + {CA-Conv}
        & $69.92 $ & $70.91 $ & $77.02 $ & $85.23 $ & $76.24 $ & $65.42 $ & $74.12 $ 
    \\
    \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/mpjpe_receptive_field_tagn.tex <==
\begin{table*}[t!]
  \caption{Effect of receptive field on $\text{MPJPE}_{\leq 0.1}$ of VP3D models trained with and without TAGN. The mean and standard deviations across $5$ random runs are reported.}
  \label{tab:supp_mpjpe-tagn-receptive-field}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}c|l|cccccc|c@{}}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Receptive \\ Field \end{tabular}} & \multicolumn{1}{c|}{ \textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impulse \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temporal-patch \\ Erasing\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Guided-patch \\ Erasing\end{tabular}} & \textbf{Cropping} & \textbf{\begin{tabular}[c]{@{}c@{}}Motion \\ Blur\end{tabular}} & \textbf{Average} \\ \midrule
    1 & VP3D\cite{pavllo2019_videopose3d}     
        & $97.80 $ & $100.06 $ & $102.80 $ & $119.24 $ & $119.00 $ & $80.39 $ & $103.22 $ 
    \\
    1 & VP3D \cite{pavllo2019_videopose3d} + {TAGN}
        & $94.98 \pm 0.09$ & $96.87 \pm 0.10$ & $94.95 \pm 0.08$ & $107.69 \pm 0.14$ & $102.16 \pm 0.62$ & $80.26 \pm 0.14$ & $96.15 \pm 0.19$ 
    \\
    \hline
    9 & VP3D\cite{pavllo2019_videopose3d}     
        & $96.61 $ & $99.11 $ & $101.95 $ & $119.03 $ & $118.85 $ & $80.92 $ & $102.74 $
    \\
    9 & VP3D \cite{pavllo2019_videopose3d} + {TAGN}
       & $93.08 \pm 0.40$ & $94.95 \pm 0.45$ & $96.69 \pm 0.21$ & $110.26 \pm 0.37$ & $107.86 \pm 0.77$ & $81.25 \pm 0.23$ & $97.35 \pm 0.40$
    \\
    \hline
    27 & VP3D\cite{pavllo2019_videopose3d}     
       & $94.27 $ & $96.64 $ & $99.32 $ & $116.54 $ & $118.08 $ & $78.14 $ & $100.50 $
    \\
    27 & VP3D \cite{pavllo2019_videopose3d} + {TAGN}
        & $86.30 \pm 0.27$ & $88.46 \pm 0.27$ & $92.57 \pm 0.33$ & $106.74 \pm 0.65$ & $107.71 \pm 0.54$ & $75.89 \pm 0.16$ & $92.94 \pm 0.37$ 
    \\
    \hline
    81 & VP3D\cite{pavllo2019_videopose3d}     
        & $93.14 $ & $95.73 $ & $97.34 $ & $114.60 $ & $120.78 $ & $76.54 $ & $99.69 $ 
    \\
    81 & VP3D \cite{pavllo2019_videopose3d} + {TAGN}
        & $84.61 \pm 0.37$ & $86.67 \pm 0.41$ & $91.36 \pm 0.20$ & $105.75 \pm 0.38$ & $106.92 \pm 0.51$ & $75.16 \pm 0.16$ & $91.74 \pm 0.34$ 
    \\
    \bottomrule
    \end{tabular}
    }
\end{table*}


==> tables/mpjpe_tagn_mean_std.tex <==
\begin{table*}[t!]
  \caption{Comparison between various baselines trained with TAGN. The mean and standard deviation across $5$ random runs are reported.}
  \label{tab:supp_mpjpe-tagn}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l|cccccc|c@{}}
    \toprule
    \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gaussian \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impulse \\ Noise\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temporal-patch \\ Erasing\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Guided-patch \\ Erasing\end{tabular}} & \textbf{Cropping} & \textbf{\begin{tabular}[c]{@{}c@{}}Motion \\ Blur\end{tabular}} & \textbf{Average} \\ \midrule
    \hline
    VP3D\cite{pavllo2019_videopose3d}/H36M+\textit{TAGN} ($\sigma=0.05; p=k=20\%$)  
         & $91.73 \pm 0.30$ & $94.12 \pm 0.32$ & $96.08 \pm 0.38$ & $112.72 \pm 0.56$ & $117.23 \pm 1.09$ & $76.54 \pm 0.24$ & $98.07 \pm 0.48$ 
    \\
    VP3D\cite{pavllo2019_videopose3d}/H36M+\textit{TAGN} ($\sigma=0.1; p=k=30\%$) 
         & $88.44 \pm 0.35$ & $90.69 \pm 0.35$ & $93.56 \pm 0.13$ & $108.95 \pm 0.22$ & $114.30 \pm 0.68$ & $75.38 \pm 0.09$ & $95.22 \pm 0.30$ 
    \\
    VP3D\cite{pavllo2019_videopose3d}/H36M+\textit{TAGN} ($\sigma=0.3; p=k=50\%$) 
         & $86.30 \pm 0.27$ & $88.46 \pm 0.27$ & $92.57 \pm 0.33$ & $106.74 \pm 0.65$ & $107.71 \pm 0.54$ & $75.89 \pm 0.16$ & $92.94 \pm 0.37$ 
    \\

    \hline
    PoseFormer\cite{zheng2021_poseformer}/H36M+\textit{TAGN} ($\sigma=0.3; p=k=50\%$) 
        & $102.24 \pm 4.03$ & $104.78 \pm 4.13$ & $113.80 \pm 3.67$ & $129.33 \pm 3.67$ & $148.39 \pm 7.11$ & $88.70 \pm 4.31$ & $114.54 \pm 4.49$ \\
    
    SRNet\cite{zeng2020_srnet}/H36M+\textit{TAGN} ($\sigma=0.3; p=k=50\%$)
         & $91.68 \pm 1.32$ & $94.04 \pm 1.49$ & $96.16 \pm 0.82$ & $111.94 \pm 0.90$ & $117.28 \pm 3.18$ & $78.70 \pm 0.59$ & $98.30 \pm 1.38$ 
        \\
    
    Attention3DHP\cite{liu2020_attention}/H36M+\textit{TAGN} ($\sigma=0.3; p=k=50\%$) 
        & $92.05 \pm 0.77$ & $93.94 \pm 0.90 $ & $100.48 \pm 1.12 $ & $115.08 \pm 1.13$ & $112.80 \pm 1.52$ & $84.35 \pm 0.81$ & $99.78 \pm 1.04$ \\
    
    Pose3D-RIE\cite{shan2021improving}/H36M+\textit{TAGN} ($\sigma=0.3; p=k=50\%$) 
         & $92.14 \pm 1.15$   & $101.34 \pm 0.23$ & $105.45 \pm 1.13$  & $115.31 \pm 0.34$  & $104.42 \pm 0.12$  & $92.40 \pm 1.62$  & $101.84 \pm 0.68$ \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

